Discovery of Visual Semantics by Unsupervised and Self-Supervised Representation Learning

The success of deep learning in computer vision is rooted in the ability of deep networks to scale up model complexity as demanded by challenging visual tasks. As complexity is increased, so is the need for large amounts of labeled data to train the model. This is associated with a costly human annotation effort. To address this concern, with the long-term goal of leveraging the abundance of cheap unlabeled data, we explore methods of unsupervised "pre-training." In particular, we propose to use self-supervised automatic image colorization. We show that traditional methods for unsupervised learning, such as layer-wise clustering or autoencoders, remain inferior to supervised pre-training. In search for an alternative, we develop a fully automatic image colorization method. Our method sets a new state-of-the-art in revitalizing old black-and-white photography, without requiring human effort or expertise. Additionally, it gives us a method for self-supervised representation learning. In order for the model to appropriately re-color a grayscale object, it must first be able to identify it. This ability, learned entirely self-supervised, can be used to improve other visual tasks, such as classification and semantic segmentation. As a future direction for self-supervision, we investigate if multiple proxy tasks can be combined to improve generalization. This turns out to be a challenging open problem. We hope that our contributions to this endeavor will provide a foundation for future efforts in making self-supervision compete with supervised pre-training.

==> include/chp2/sec0-abstract.tex <==
%auto-ignore
\begin{abstract}
We develop a fully automatic image colorization system.  Our approach
leverages recent advances in deep networks, exploiting both low-level and
semantic representations.  As many scene elements naturally appear according to
multimodal color distributions, we train our model to predict per-pixel color
histograms.  This intermediate output can be used to automatically generate a
color image, or further manipulated prior to image formation.  On both fully
and partially automatic colorization tasks, we outperform existing methods.
We also explore colorization as a vehicle for self-supervised visual
representation learning.
% keywords can be omitted from review copy
%\keywords{
%  Automatic colorization, convolutional neural networks, hypercolumns, deep learning.
%}
\end{abstract}


==> include/chp3/sec0-abstract.tex <==
We investigate and improve self-supervision as a drop-in replacement for ImageNet pretraining, focusing on automatic colorization as the proxy task.  Self-supervised training has been shown to be more promising for utilizing unlabeled data than other, traditional unsupervised learning methods. We build on this success and evaluate the ability of our self-supervised network in several contexts. On VOC segmentation and classification tasks, we present results that are state-of-the-art among methods not using ImageNet labels for pretraining representations.

Moreover, we present the first in-depth analysis of self-supervision via colorization, concluding that formulation of the loss, training details and network architecture play important roles in its effectiveness. This investigation is further expanded by revisiting the ImageNet pretraining paradigm, asking questions such as: How much training data is needed? How many labels are needed? How much do features change when fine-tuned? We relate these questions back to self-supervision by showing that colorization provides a similarly powerful supervisory signal as various flavors of ImageNet pretraining.


==> include/chp3/tab-voc2012seg.tex <==
\begin{table*}
\centering
    {\small
    \begin{tabular*}{\textwidth}{l|@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}c@{\ab}|c}
        \toprule
        Initialization & bkg  & aero & bike & bird & boat & bottle & bus  & car  & cat  & chair & cow  & tabl & dog  & horse & mbike & person & plant & sheep & sofa & train & tv   & \%mIU \\ \midrule
        Random         & 84.7 & 50.2 & 22.1 & 27.0 & 29.0 & 21.2 & 62.5 & 52.0 & 46.7 & 7.9 & 13.9 & 18.5 & 33.3 & 25.8 & 42.2 & 51.7 & 13.7 & 33.3 & 19.3 & 52.0 & 30.8\, &  \textbf{35.1}\cmt{a156} \\
        Colorization   & 89.8 & 73.9 & 27.3 & 59.1 & 51.3 & 50.6 & 77.1 & 71.1 & 70.0 & 26.7 & 47.1 & 39.2 & 58.8 & 60.8 & 61.3 & 73.2 & 31.7 & 57.9 & 30.3 & 66.4 & 52.3\, & \textbf{56.0}\cmt{a138} TODO update \\
        Classification & 91.5 & 83.1 & 37.1 & 77.6 & 60.7 & 64.5 & 84.9 & 78.9 & 83.1 & 32.7 & 68.7 & 41.9 & 74.7 & 72.4 & 74.5 & 76.3 & 42.4 & 74.0 & 41.4 & 76.6 & 59.7\, & \textbf{66.5}\cmt{a135} \\
        \bottomrule
    \end{tabular*}
    }
    \caption{
        \small
        [TODO if kept, I should chagne the random/classification to ResNet as well] \textbf{VOC 2012 Segmentation (val, grayscale).} Using colorization as a pretraining offers a significant improvement over random initialization, roughly two-thirds bridging the gap to classification-based methods.
        %For many classes, the improvement   (e.g. bird $27.0 \rightarrow 59.1$, chair $7.9 \rightarrow 26.7$).
        In particular, our method is only 3.1 points shy of classification-based performance on the \emph{person} class (73.2\% vs.\ 76.3\% mIU).
    }\label{tab:voc2012seg}
\end{table*}


==> include/chp4/tab-dist-dropout.tex <==
\begin{table}
    % This doesn't fit in
    \newcommand{\xa}[3]{$\num[round-mode=places,round-precision=1]{#1}\pm\num[round-mode=places,round-precision=1]{#2}$}
    \newcommand{\xb}[2]{$\num[round-mode=places,round-precision=1]{#1}\phantom{^{}\pm0.0}$}
    %\xa{48.86}{pc131,pc138,pc139,pc140-average of 139/140}
    \newcommand{\tb}{\textbf}
    \begin{center}
        \begin{tabular*}{\linewidth}{lccc|@{\quad\,\,}r}
            \toprule Samples 
            & Data Augmentation
            & Student Dropout
            & Teacher Dropout
            & \textit{Task-Compress}
            \\ \midrule
            40,000 & &  &  & \xa{40.808}{0.399769933837}{pc371} \\
            40,000 & & \cmark & & \xa{37.538}{0.155228863295}{pc372} \\
            40,000 & & & \cmark & \xa{40.962}{0.841080257764}{pc373} \\
            40,000 & & \cmark & \cmark & \xa{37.988}{0.30695}{pc294} \\ \midrule
            40,000 & \cmark & &  & \xa{41.834}{0.376223337926}{pc374} \\
            40,000 & \cmark & \cmark & & \xa{36.742}{0.277445490142}{pc375} \\
            40,000 & \cmark & & \cmark & ..\cmt{pc376} \\
            40,000 & \cmark & \cmark & \cmark & \xa{36.966}{0.4449}{pc377} \\
        \bottomrule
        \end{tabular*}
    \end{center}
    \caption[Distillation and dropout]{
        \textbf{Distillation and dropout.}
        Ablation study of dropout and data augmentation impact on model
        distillation results.
        Dropout in the student is the most effective method for regularizing
        model distillation when data is scarce.
    }
    \label{tab:dist-dropout}
\end{table}


% Experiments:
% cat pc294/res-*.txt | python mean.py

